Class Distribution Monitoring for Concept Drift Detection

We introduce Class Distribution Monitoring (CDM), an effective concept-drift detection scheme that monitors the class-conditional distributions of a datastream. In particular, our solution leverages multiple instances of an online and nonparametric change-detection algorithm based on QuantTree. CDM reports a concept drift after detecting a distribution change in any class, thus identifying which classes are affected by the concept drift. This can be precious information for diagnostics and adaptation. Our experiments on synthetic and real-world datastreams show that when the concept drift affects a few classes, CDM outperforms algorithms monitoring the overall data distribution, while achieving similar detection delays when the drift affects all the classes. Moreover, CDM outperforms comparable approaches that monitor the classification error, particularly when the change is not very apparent. Finally, we demonstrate that CDM inherits the properties of the underlying change detector, yielding an effective control over the expected time before a false alarm, or Average Run Length (ARL$_0$).

==> figures/gaussian_setting/gaussian_setting.tex <==
% \begin{figure}
%     \centering
    % \begin{minipage}[c]{.4\columnwidth}
    \begin{tikzpicture}
    \begin{axis}[
        width=0.8\columnwidth,
        height=0.5\columnwidth,
        scale only axis,
        xmin=-2, xmax=4,
        ymin=-2, ymax=2,
        axis line style={draw=none},
        tick style={draw=none},
        xticklabels={,,},
        yticklabels={,,}
        ]
    %,
    \draw[color=colorblind1, thin, ->](-2,0) -- (4,0);
    \draw[color=colorblind1, thin, ->](0,-2) -- (0,2);
    %
    \filldraw[color=colorblind2, fill=none, very thick](0,0) circle (1.5);
    \node [colorblind2] at (0,-.035) {\textbullet};
    \node[text width=1cm] at (0.09,0.3) {$\mu_0^1$};
    \node[text width=1cm] at (-1.3,1.25) {$\phi_0^1$};
    %
    \filldraw[color=colorblind3, fill=none, very thick](2,0) circle (1.5);
    \node [colorblind3] at (2,-.035) {\textbullet};
    \node[text width=1cm] at (2.09,0.3) {$\mu_0^2$};
    \node[text width=1cm] at (3.6,1.25) {$\phi_0^2$};
    %
    \draw[color=colorblind8, thick, ->](2,0) -- (1.8,-0.7);
    \node[text width=1cm] at (1.8,-0.7) {$\mu_1^2$};
    \node [colorblind8] at (1.79,-0.75) {\textbullet};
    \draw[colorblind8, thick, dashed] (0.5,-1.0) -- (0.5,1.0) -- (2.5,1.0) -- (2.5,-1.0) -- cycle;
    \end{axis}
    \end{tikzpicture}
    % \end{minipage}
% \caption{Hello, world!}
% \end{figure}

% \begin{tikzpicture}
%     \begin{axis}[
%         width=0.9\columnwidth,
%         height=0.5\columnwidth,
%         scale only axis,
%         ]
%         \coordinate (c1) at (rel axis cs:0.51,0.535);
%         \coordinate (c2) at (rel axis cs:0.645,0.93);
%     \end{axis}
% \end{tikzpicture}

==> figures/heatmaps/heatmaps.tex <==
% \newcommand{\EXT}{.eps}
\newcommand{\EXT}{.pdf}

\begin{figure*}
\centering
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=\textwidth]{figures/heatmaps/heatmap_ecdd\EXT}
  \caption{}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=\textwidth]{figures/heatmaps/heatmap_cdm\EXT}
  \caption{}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=\textwidth]{figures/heatmaps/heatmap_diff\EXT}
  \caption{}
  \label{fig:sub-third}
\end{subfigure}

\caption{
Results of the experiment on synthetic data. The blue dot represents the pre-change mean $\mu_0^2$. (\subref{fig:sub-first},\subref{fig:sub-second}) report, at each coordinate $\overline{\mu}$, the average detection delay achieved by ECDD and CDM, respectively, when $\mu_0^2 \to \overline{\mu}$. In (\subref{fig:sub-first}) the contour lines indicate the difference in classification error $p_1 - p_0$ before and after the change, and in (\subref{fig:sub-second}) the change magnitude $\skl(\phi_0^2, \phi_1^2)$. 
(\subref{fig:sub-third}) report the difference between the detection delay achieved over synthetic data by ECDD and CDM, with contour lines.
% Results of the experiment on synthetic data. The blue dot represents the mean $\mu_0^2$ of $\phi_0^2$ before the change. At each coordinate $\overline{\mu}$, the color coded values represent the average (difference of) detection delay achieved when $\mu_0^2 \to \overline{\mu}$. 
% (\subref{fig:sub-first})~Detection delay achieved by ECDD on the considered synthetic scenario. Contour lines refer to the difference in classification error $p_1 - p_0$ before and after the change.
% (\subref{fig:sub-second})~Detection delay achieved by CDM on the considered synthetic scenario. Contour lines represent the change magnitude measured as $\skl(\phi_0^2, \phi_1^2)$.
% (\subref{fig:sub-third})~Difference between the detection delay achieved over synthetic data by ECDD and CDM, with contour lines.
}
\label{fig:heatmaps}
\end{figure*}

==> figures/insects_arl0.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{png_figs/spider_512.png}
    \caption{Average Run Length ($\arl{0}$) of the considered methods for different concepts.}
    \label{fig:arl0_insects}
\end{figure}

==> figures/insects_delay.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{png_figs/insects_scatter_512.png}
    \caption{Detection delay of the considered methods for different concepts (i.e., different starting classification errors $p_0$).}
    \label{fig:delay_insects}
\end{figure}

==> figures/insects_delay/ins_del_conceptA.tex <==
\addplot [only marks, mark=\cdmMarker, mark size = 2pt,
mark options={line width=.2pt, draw=cdm_c, fill = cdm_c, opacity=.4},]
table [x=dp0, y=cdm,] {figures/insects_delay/data/ins_del_scatter_conceptA_cdm.txt};
%
\addplot [only marks, mark=\ecddMarker, mark size = 2pt, mark options={line width=.2pt, draw=ecdd_c, fill = ecdd_c, opacity=.4},]
table [x=dp0, y=ecdd,] {figures/insects_delay/data/ins_del_scatter_conceptA_ecdd.txt};
%
\addplot [color=cdm_c, solid, line width=1pt, mark=none, mark size = 1.5pt, mark options={solid},]
table [x=dp0, y=cdm,]
{figures/insects_delay/data/ins_del_plot_conceptA.txt};
%
\addplot [color=ecdd_c, solid, line width=1pt, mark=none, mark size = 1.5pt, mark options={solid},]
table [x=dp0, y=ecdd,]
{figures/insects_delay/data/ins_del_plot_conceptA.txt};
%

==> figures/insects_delay/ins_del_conceptB.tex <==
\addplot [only marks, mark=\cdmMarker, mark size = 2pt,
mark options={line width=.2pt, draw=cdm_c, fill = cdm_c, opacity=.4},]
table [x=dp0, y=cdm,] {figures/insects_delay/data/ins_del_scatter_conceptB_cdm.txt};
% \addlegendentry{CDM (ours)}
%
\addplot [only marks, mark=\ecddMarker, mark size = 2pt, mark options={line width=.2pt, draw=ecdd_c, fill = ecdd_c, opacity=.4},]
table [x=dp0, y=ecdd,] {figures/insects_delay/data/ins_del_scatter_conceptB_ecdd.txt};
% \addlegendentry{ECDD [4]}
%
\addplot [color=cdm_c, solid, line width=1pt, mark=none, mark size = 1.5pt, mark options={solid},]
table [x=dp0, y=cdm,]
{figures/insects_delay/data/ins_del_plot_conceptB.txt};
%
\addplot [color=ecdd_c, solid, line width=1pt, mark=none, mark size = 1.5pt, mark options={solid},]
table [x=dp0, y=ecdd,]
{figures/insects_delay/data/ins_del_plot_conceptB.txt};
%

==> figures/insects_delay/ins_del_conceptC.tex <==
\addplot [only marks, mark=\cdmMarker, mark size = 2pt,
mark options={line width=.2pt, draw=cdm_c, fill = cdm_c, opacity=.4},]
table [x=dp0, y=cdm,] {figures/insects_delay/data/ins_del_scatter_conceptC_cdm.txt};
% \addlegendentry{CDM}
%
\addplot [only marks, mark=\ecddMarker, mark size = 2pt, mark options={line width=.2pt, draw=ecdd_c, fill = ecdd_c, opacity=.4},]
table [x=dp0, y=ecdd,] {figures/insects_delay/data/ins_del_scatter_conceptC_ecdd.txt};
% \addlegendentry{ECDD}
%
\addplot [color=cdm_c, solid, line width=1pt, mark=none, mark size = 1.5pt, mark options={solid},]
table [x=dp0, y=cdm,]
{figures/insects_delay/data/ins_del_plot_conceptC.txt};
%
\addplot [color=ecdd_c, solid, line width=1pt, mark=none, mark size = 1.5pt, mark options={solid},]
table [x=dp0, y=ecdd,]
{figures/insects_delay/data/ins_del_plot_conceptC.txt};
%

==> figures/insects_delay/ins_del_conceptD.tex <==
\addplot [only marks, mark=\cdmMarker, mark size = 2pt,
mark options={line width=.2pt, draw=cdm_c, fill = cdm_c, opacity=.4},]
table [x=dp0, y=cdm,] {figures/insects_delay/data/ins_del_scatter_conceptD_cdm.txt};
%
\addplot [only marks, mark=\ecddMarker, mark size = 2pt, mark options={line width=.2pt, draw=ecdd_c, fill = ecdd_c, opacity=.4},]
table [x=dp0, y=ecdd,] {figures/insects_delay/data/ins_del_scatter_conceptD_ecdd.txt};
%
\addplot [color=cdm_c, solid, line width=1pt, mark=none, mark size = 1.5pt, mark options={solid},]
table [x=dp0, y=cdm,]
{figures/insects_delay/data/ins_del_plot_conceptD.txt};
%
\addplot [color=ecdd_c, solid, line width=1pt, mark=none, mark size = 1.5pt, mark options={solid},]
table [x=dp0, y=ecdd,]
{figures/insects_delay/data/ins_del_plot_conceptD.txt};
%

==> figures/insects_delay/ins_del_conceptE.tex <==
\addplot [only marks, mark=\cdmMarker, mark size = 2pt,
mark options={line width=.2pt, draw=cdm_c, fill = cdm_c, opacity=.4},]
table [x=dp0, y=cdm,] {figures/insects_delay/data/ins_del_scatter_conceptE_cdm.txt};
%
\addplot [only marks, mark=\ecddMarker, mark size = 2pt, mark options={line width=.2pt, draw=ecdd_c, fill = ecdd_c, opacity=.4},]
table [x=dp0, y=ecdd,] {figures/insects_delay/data/ins_del_scatter_conceptE_ecdd.txt};
%
\addplot [color=cdm_c, solid, line width=1pt, mark=none, mark size = 1.5pt, mark options={solid},]
table [x=dp0, y=cdm,]
{figures/insects_delay/data/ins_del_plot_conceptE.txt};
%
\addplot [color=ecdd_c, solid, line width=1pt, mark=none, mark size = 1.5pt, mark options={solid},]
table [x=dp0, y=ecdd,]
{figures/insects_delay/data/ins_del_plot_conceptE.txt};
%

==> figures/insects_delay/ins_del_conceptF.tex <==
\addplot [only marks, mark=\cdmMarker, mark size = 2pt,
mark options={line width=.2pt, draw=cdm_c, fill = cdm_c, opacity=.4},]
table [x=dp0, y=cdm,] {figures/insects_delay/data/ins_del_scatter_conceptF_cdm.txt};
\addlegendentry{CDM}
%
\addplot [only marks, mark=\ecddMarker, mark size = 2pt,
mark options={line width=.2pt, draw=ecdd_c, fill = ecdd_c, opacity=.4},]
table [x=dp0, y=ecdd,] {figures/insects_delay/data/ins_del_scatter_conceptF_ecdd.txt};
\addlegendentry{ECDD}
%
\addplot [color=cdm_c, solid, line width=1pt, mark=none, mark size = 1.5pt, mark options={solid},]
table [x=dp0, y=cdm,]
{figures/insects_delay/data/ins_del_plot_conceptF.txt};
%
\addplot [color=ecdd_c, solid, line width=1pt, mark=none, mark size = 1.5pt, mark options={solid},]
table [x=dp0, y=ecdd,]
{figures/insects_delay/data/ins_del_plot_conceptF.txt};
%

==> figures/insects_delay/insects_delay_main.tex <==
\begin{tikzpicture}
\begin{groupplot}[
    % group style={group size=3 by 2, horizontal sep=1.5cm, vertical sep=1.5cm},
    group style={group size=3 by 2, horizontal sep=.05cm, vertical sep=1.5cm},
    width=.29\textwidth,
    height=.15\textwidth,
    title style = {font=\small,
        at={(0.5, 0.92)},
    },
    scale only axis,
    ymajorgrids,
    xlabel style = {font=\footnotesize},
    ylabel style = {font=\footnotesize},
    xticklabel style = {font = \scriptsize},
    yticklabel style = {font = \scriptsize},
    xtick = {-0.1,0,...,0.5},
    % yticklabels={,,},
    % minor xtick = {1,3,...,11},
    xmin=-0.075,
    xmax=0.4,
    %xlabel style = {align=center},
    %xlabel style = {anchor = near ticklabel, at = {(0.5,0.04)}},
    %ylabel style = {anchor = near ticklabel, at = {(0.15,0.5)}},
    %yticklabel style = {font = \small},
    % legend columns=7, 
    % legend style={at={(0,.-05)},   % where in the figure
    % 	anchor=north east,          % which corner is "at" referring to
    % 	font=\small,                
    % 	legend cell align=left},
    %reverse legend
]
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
%
\nextgroupplot[title={Concept A ($p_0 = 0.227$)},
ytick = {0,50,...,600}, ymin=0, ymax=500, ylabel={Detection delay},
xlabel={$p_1 - p_0$},
legend style={at={($(0,0)+(0cm,0cm)$)},legend columns=-1,fill=none,draw=black,anchor=center,align=center, font=\small,},]
\input{figures/insects_delay/ins_del_conceptA}
%
\nextgroupplot[title={Concept B ($p_0 = 0.304$)},
ytick = {0,50,...,600}, ymin=0, ymax=500, ylabel={}, yticklabels={,,},
xlabel={$p_1 - p_0$},
legend style={at={($(0.6,0.8)+(0cm,0cm)$)},legend columns=-1,fill=none,draw=black,anchor=center,align=center, font=\small,},]
\input{figures/insects_delay/ins_del_conceptB}
%
\nextgroupplot[title={Concept C ($p_0 = 0.173$)},
ytick = {0,50,...,600}, ymin=0, ymax=500, ylabel={}, yticklabels={,,},
xlabel={$p_1 - p_0$},
legend style={at={($(0,0)+(0cm,0cm)$)},legend columns=-1,fill=none,draw=black,anchor=center,align=center, font=\small, 
%legend to name = grouplegend,
},]
\input{figures/insects_delay/ins_del_conceptC}
%
\nextgroupplot[title={Concept D ($p_0 = 0.212$)},
ytick = {0,50,...,600}, ymin=0, ymax=500, ylabel={Detection delay},
xlabel={$p_1 - p_0$},
legend style={at={($(0,0)+(0cm,0cm)$)},legend columns=-1,fill=none,draw=black,anchor=center,align=center, font=\small,},]
\input{figures/insects_delay/ins_del_conceptD}
%
\nextgroupplot[title={Concept E ($p_0 = 0.165$)},
ytick = {0,50,...,600}, ymin=0, ymax=500, ylabel={}, yticklabels={,,},
xlabel={$p_1 - p_0$},
legend style={at={($(0,0)+(0cm,0cm)$)},legend columns=-1,fill=none,draw=black,anchor=center,align=center, font=\small,},]
\input{figures/insects_delay/ins_del_conceptE}
%
\nextgroupplot[title={Concept F ($p_0 = 0.170$)},
ytick = {0,50,...,600}, ymin=0, ymax=500, ylabel={}, yticklabels={,,},
xlabel={$p_1 - p_0$},
legend style={at={($(0,0)+(0cm,0cm)$)},legend columns=-1,fill=none,draw=black,anchor=center,align=center, font=\small, 
legend to name = grouplegend,
},]
\input{figures/insects_delay/ins_del_conceptF}
%
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
\end{groupplot}
%
\node at ($(group c3r2) + (1.2cm,.9cm)$) {\ref{grouplegend}}; 
% \node [right] at ($(my plots c1r1.east)!.5!(my plots c1r2.east)$)     {\ref{fig:my plots:grouplegend}};
% \draw ($(group c1r1.north west) + (0cm,.75cm)$) -- ($(group c2r1.north east) + (0cm,.75cm)$);
% \node[align=center] at ($(group c1r1.north west)!.5!(group c2r1.north east) + (0cm,1cm)$) {AUC};
% \draw ($(group c3r1.north west) + (0cm,.75cm)$) -- ($(group c4r1.north east) + (0cm,.75cm)$);
% \node[align=center] at ($(group c3r1.north west)!.5!(group c4r1.north east) + (0cm,1cm)$) {FPR};
\end{tikzpicture}%

==> figures/insects_delay/insects_delay_tikz.tex <==
\begin{figure*}[t!]
    % \hspace{-1cm}
    \input{figures/insects_delay/insects_delay_main}
    % \input{figures/insects_delay/insects_poster}
    \caption{
    Detection delay achieved by ECDD and CDM on the INSECTS dataset~\cite{souza2020challenges} for each of the $6$ stationary concepts, plotted against the difference $p_1-p_0$, where $p_0,p_1$ are the error rates of $\mathcal{K}$ before and after the drift. Each dot is the average of $1000$ realizations of the same change $\phi_0 \to \phi_1$ i.e., thus with the same affected classes.
    }
    \label{fig:delay_insects}
% \vspace{-0.3cm}
\end{figure*}

==> figures/insects_delay/insects_poster.tex <==
\begin{tikzpicture}
\begin{groupplot}[
    % group style={group size=3 by 2, horizontal sep=1.5cm, vertical sep=1.5cm},
    group style={group size=2 by 1, horizontal sep=.05cm},
    width=.45\textwidth,
    height=.2\textwidth,
    title style = {font=\small,
        at={(0.5, 0.94)},
    },
    scale only axis,
    ymajorgrids,
    xlabel style = {font=\footnotesize},
    ylabel style = {font=\footnotesize},
    xticklabel style = {font = \scriptsize},
    yticklabel style = {font = \scriptsize},
    xtick = {-0.1,0,...,0.5},
    % yticklabels={,,},
    % minor xtick = {1,3,...,11},
    xmin=-0.075,
    xmax=0.4,
    %xlabel style = {align=center},
    %xlabel style = {anchor = near ticklabel, at = {(0.5,0.04)}},
    %ylabel style = {anchor = near ticklabel, at = {(0.15,0.5)}},
    %yticklabel style = {font = \small},
    % legend columns=7, 
    % legend style={at={(0,.-05)},   % where in the figure
    % 	anchor=north east,          % which corner is "at" referring to
    % 	font=\small,                
    % 	legend cell align=left},
    %reverse legend
]
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
%
\nextgroupplot[title={Concept A ($p_0 = 0.227$)},
ytick = {0,50,...,600}, ymin=0, ymax=500, ylabel={Detection delay},
xlabel={$p_1 - p_0$},
legend style={at={($(0,0)+(0cm,0cm)$)},legend columns=-1,fill=none,draw=black,anchor=center,align=center, font=\small,},]
\input{figures/insects_delay/ins_del_conceptA}
%
\nextgroupplot[title={Concept B ($p_0 = 0.304$)},
ytick = {0,50,...,600}, ymin=0, ymax=500, ylabel={}, yticklabels={,,},
xlabel={$p_1 - p_0$},
legend style={at={($(0,0)+(0cm,0.1cm)$)},legend columns=-1,fill=none,draw=black,anchor=center,align=center, font=\small, 
legend to name = grouplegend,
},]
\input{figures/insects_delay/ins_del_conceptB}
%
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
\end{groupplot}
%
\node at ($(group c2r1) + (1.2cm,.9cm)$) {\ref{grouplegend}}; 
% \node [right] at ($(my plots c1r1.east)!.5!(my plots c1r2.east)$)     {\ref{fig:my plots:grouplegend}};
% \draw ($(group c1r1.north west) + (0cm,.75cm)$) -- ($(group c2r1.north east) + (0cm,.75cm)$);
% \node[align=center] at ($(group c1r1.north west)!.5!(group c2r1.north east) + (0cm,1cm)$) {AUC};
% \draw ($(group c3r1.north west) + (0cm,.75cm)$) -- ($(group c4r1.north east) + (0cm,.75cm)$);
% \node[align=center] at ($(group c3r1.north west)!.5!(group c4r1.north east) + (0cm,1cm)$) {FPR};
\end{tikzpicture}%

==> figures/linear_delay.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{png_figs/HEATMAP_Difference.png}
    \caption{Difference between the detection delay of ECDD and QT-EWMA-CDS. Vertical contour plots refer to the increase in classification error.}
    \label{fig:delay_linear}
\end{figure}

==> tables/table_insects_delay_all.tex <==
\begin{table}[t!]
\centering
\caption{Average detection delays on the 6 concepts (each representing an initial distribution $\phi_0$) of the INSECTS dataset~\cite{souza2020challenges}. For each concept we report the initial error rate $p_0$ of the classifier. \di{Il p0 è un'informazione ripetuta (dato che è anche nella tabella di ARL0. Togliere?}
}\label{tab:insects_delays_concepts}
\resizebox{\columnwidth}{!}{  
\begin{tabular}{c|cccc} 
\hline
Concept  & ECDD~\cite{ross2012exponentially} & Scan-B~\cite{li2015m} & QT-EWMA~\cite{frittoli2021change} & CDM (ours)\\
\hline
1      & $260.00$ & $\mathbf{159.48}$ & $220.20$ & $167.92$          \\  
2      & $116.97$ & $66.94$  & $109.71$ & $\mathbf{56.79}$           \\  
3      & $200.70$ & $184.54$ & $237.40$ & $\mathbf{173.34}$          \\  
4      & $156.06$ & $129.18$ & $162.11$ & $\mathbf{101.92}$          \\  
5      & $175.06$ & $178.75$ & $211.15$ & $\mathbf{158.36}$          \\  
6      & $178.52$ & $183.56$ & $223.50$ & $\mathbf{157.22}$          \\  
\hline
\hline
Changed species &  &  & & \\
\hline
A          & $207.98$ & $212.53$ & $267.73$ & $\textbf{195.45}$ \\  
B          & $245.85$ & $162.58$ & $195.44$ & $\textbf{124.92}$ \\  
C          & $264.27$ & $224.99$ & $278.57$ & $\textbf{204.00}$ \\  
D          & $224.91$ & $235.87$ & $265.96$ & $\textbf{196.74}$ \\  
A, B       & $198.17$ & $131.71$ & $174.80$ & $\textbf{114.44}$ \\  
A, C       & $172.62$ & $169.87$ & $223.50$ & $\textbf{160.98}$ \\  
A, D       & $165.77$ & $163.63$ & $221.66$ & $\textbf{145.82}$ \\  
B, C       & $163.66$ & $126.56$ & $167.55$ & $\textbf{112.18}$ \\  
B, D       & $176.53$ & $119.41$ & $154.95$ & $\textbf{106.49}$ \\  
C, D       & $210.04$ & $169.88$ & $218.90$ & $\textbf{153.51}$ \\  
A, B, C    & $139.29$ & $115.01$ & $152.91$ & $\textbf{103.60}$ \\  
A, B, D    & $148.03$ & $103.24$ & $141.09$ & $\textbf{98.89}$  \\  
A, C, D    & $144.81$ & $134.83$ & $183.41$ & $\textbf{131.38}$ \\  
B, C, D    & $132.36$ & $\textbf{96.92}$  & $136.90$ & $98.57$  \\  
A, B, C, D & $122.38$ & $\textbf{88.86}$  & $128.04$ & $91.44$  \\  
\hline
\hline
Avg. rank       & $2.416$  & $2.356$  & $3.524$  & $\mathbf{1.704}$           \\ 
Nemenyi-p      & $6.95\cdot10^{-06}$ & $1.44\cdot10^{-01}$ & $5.18\cdot10^{-17}$         & -- \\  
Dunn-p          & $2.43\cdot10^{-07}$ & $2.01\cdot10^{-02}$ & $6.40\cdot10^{-19}$       & -- \\  
\hline

\end{tabular}
}
\end{table}

==> tables/table_insects_delay_concept.tex <==
\begin{table}[t!]
\centering
\caption{Average detection delays on the 6 concepts (each representing an initial distribution $\phi_0$) of the INSECTS dataset~\cite{souza2020challenges}. For each concept we report the initial error rate $p_0$ of the classifier. \di{Il p0 è un'informazione ripetuta (dato che è anche nella tabella di ARL0. Togliere?}
}\label{tab:insects_delays_concepts}
\resizebox{\columnwidth}{!}{  
\begin{tabular}{c|cccc} 
\hline
Concept ($p_0$) & ECDD~\cite{ross2012exponentially} & Scan-B~\cite{li2015m} & QT-EWMA~\cite{frittoli2021change} & CDM (ours)\\
\hline
1 ($0.227$)      & $260.00$ & $\mathbf{159.48}$ & $220.20$ & $167.92$          \\  
2 ($0.304$)      & $116.97$ & $66.94$  & $109.71$ & $\mathbf{56.79}$           \\  
3 ($0.173$)      & $200.70$ & $184.54$ & $237.40$ & $\mathbf{173.34}$          \\  
4 ($0.212$)      & $156.06$ & $129.18$ & $162.11$ & $\mathbf{101.92}$          \\  
5 ($0.165$)      & $175.06$ & $178.75$ & $211.15$ & $\mathbf{158.36}$          \\  
6 ($0.170$)      & $178.52$ & $183.56$ & $223.50$ & $\mathbf{157.22}$          \\  
\hline 
Avg. rank       & $2.416$  & $2.356$  & $3.524$  & $\mathbf{1.704}$           \\ 
Nemenyi-p      & $6.95\cdot10^{-06}$ & $1.44\cdot10^{-01}$ & $5.18\cdot10^{-17}$         & -- \\  
Dunn-p          & $2.43\cdot10^{-07}$ & $2.01\cdot10^{-02}$ & $6.40\cdot10^{-19}$       & -- \\  
\hline
\end{tabular}
}
\end{table}
